FOREST: An Interactive Multi-tree Synthesizer for Regular Expressions

Form validators based on regular expressions are often used on digital forms to prevent users from inserting data in the wrong format. However, writing these validators can pose a challenge to some users. We present FOREST, a regular expression synthesizer for digital form validations. FOREST produces a regular expression that matches the desired pattern for the input values and a set of conditions over capturing groups that ensure the validity of integer values in the input. Our synthesis procedure is based on enumerative search and uses a Satisfiability Modulo Theories (SMT) solver to explore and prune the search space. We propose a novel representation for regular expressions synthesis, multi-tree, which induces patterns in the examples and uses them to split the problem through a divide-and-conquer approach. We also present a new SMT encoding to synthesize capture conditions for a given regular expression. To increase confidence in the synthesized regular expression, we implement user interaction based on distinguishing inputs. We evaluated FOREST on real-world form-validation instances using regular expressions. Experimental results show that FOREST successfully returns the desired regular expression in 72% of the instances and outperforms REGEL, a state-of-the-art regular expression synthesizer.

==> figures/node_comparison_encoding.tex <==
\begin{figure}[t]
    \centering
    \begin{tikzpicture}
        \begin{axis}[grid=major,
                    xlabel = {\small K-tree enumerator (s)},
                    ylabel = {\small Multi-tree enumerator (s)},
                    xmax = 15 ,ymax = 15,
                    width=.60\linewidth, height=.60\linewidth,
                    clip marker paths=true]
        \addplot[only marks,fill opacity=0.6, draw opacity = 0, color = scatter-color] table[x=KTree, y=MultiTree, col sep=comma] {data/node_comparison.csv};
        \addplot[domain=0.1:600,smooth,thin]{x};
        \end{axis}
    \end{tikzpicture}

\caption{Comparison of number of nodes between K-tree and multi-tree encodings}
\label{fig:nodes-comparison-encoding}
\end{figure}

==> figures/time_comparison_encoding.tex <==
\begin{figure}[t]
\centering
    \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \compareTimesPlot{multitree}{Multi-tree (s)}{ktree}{\(k\)-tree (s)}
         \caption{Multi-tree vs. \(k\)-tree}
         \label{fig:mt_vs_ktree}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \compareTimesPlot{nopruning}{Multi-tree w/o pruning (s)}{lines}{Line-based (s)}
         \caption{Multi-tree vs. line-based}
         \label{fig:mt_vs_lines}
     \end{subfigure}
\caption{Comparison of time performance of the synthesizer using different encodings.}
\label{fig:time-comparison-encodings}
\end{figure}


==> figures/time_comparison_resnax.tex <==
\definecolor{error-color}{HTML}{a30b00}
\begin{figure}[t]
\centering
\begin{subfigure}[b]{0.7\textwidth}

\begin{tikzpicture}
  \begin{axis}[xmode=log, ymode=log, grid=major,
                xlabel = {\small \Regel{} (s)},
                ylabel = {\small \Forest{}'s first solution (s)},
                xmax = 20000 ,ymax = 20000,
                width=.99\linewidth, height=.99\linewidth,
                clip marker paths=true]
                

  \addplot [dotted, very thick, magenta, opacity=0.8] coordinates {(0.01,3600) (3600,3600)}; % node at (1,5000) {\scriptsize{3600 second timeout}};
  
  \addplot [dotted, very thick, magenta, opacity=0.8] coordinates {(3600,0.01) (3600,3600)};
       % node [rotate=-90] at (5000,1) {\scriptsize{3600 second timeout}};
  
  \addplot [dotted, very thick, orange, opacity=0.8] coordinates {(10000,0.01) (10000,10000)};
       % node [rotate=-90] at (14000,0.5) {\scriptsize{Out of memory}};
       
       
  \addplot[only marks, mark=x, thick, fill opacity=0.5, draw opacity=0.9, color=blue] table[x=resnax, y=mt_seq, col sep=comma] {data/time_comparison_15.csv};
  
  \addplot[only marks, mark=x, thick, fill opacity=0.6, draw opacity=0.9, color=teal] table[x=resnax, y=firstforest, col sep=comma] {data/resnax_instances.csv};
  
  \addplot[only marks, mark=x, thick, fill opacity=0.6, draw opacity=0.9, color=teal] table[x=resnax, y=first-forest, col sep=comma] {data/resnax_errors_resnax.csv};
  
  
  \addplot[domain=0.1:3600,smooth,thin]{x};
  
  \end{axis}
\end{tikzpicture}

  \end{subfigure}
\caption{Comparison of time performance between \Forest{} and \Regel{}. Marks on the dotted magenta line indicate that the corresponding instance timed out after 3600 seconds, and marks on the dotted orange line mean that the synthesizer was stopped for having exceeded the 32GB memory limit.}
\label{fig:time-comparison-resnax}
\end{figure}

==> sections/ktree.tex <==
\section{\texorpdfstring{\(k\)-tree encoding}{k-tree encoding}}\label{sec:ktree}
In this section we offer a formal description of the \(k\)-tree encoding, as proposed by Chen et. al. \cite{DBLP:conf/sigsoft/ChenMF19}.
Consider a \(k\)-tree of depth \(d\). Assume each node in the \(k\)-tree is assigned a unique positive integer index consistent with level-order traversal. Let \(N\) be the set all nodes' indices, \(N = \{1, 2, ..., k^d - 1\}\).
Let \(L\) be the set of indices that correspond to leaf nodes and \(I\) the set of indices of internal nodes. Thus \(N = I \cup L\). Furthermore, let \(C(i)\) represent the indices of all children of node \(i\).

Let \(id: \Sigma \to \mathbb{N}\) be a one-to-one mapping of each terminal symbol (i.e., operators and literals) in the DSL to a positive integer.
Because the arity of some DSL operations is smaller than \(k\), there are some children nodes that cannot be assigned any symbol. We introduce the empty symbol, \(\epsilon\), with \(id(\epsilon) = 0\), which is assigned to nodes without symbols.

\paragraph{Encoding variables.}
We define an integer variable \(n_i\) for all \(i \in N\). Assigning \(n_i = id(k)\) means
that we assign the symbol~\(k\) to node \(i\).

\medskip

Next, we add constraints over these variables that ensure the generated regular expression is well-typed. All examples in the remainder of this section refer to the DSL presented in \autoref{ex:dsl} built for the problem described in \autoref{ex:1}.

\paragraph{Leaf constraints.} 
Because they have no children, the leaf nodes must be empty or assigned to a literal of the DSL.
Let \(T\) be the union of \(\epsilon\) with the set of terminal symbols in the DSL that correspond to literals.

\begin{equation}
    \bigwedge_{i \in L} \; \bigvee_{p \in T} n_i = id(p)
\end{equation}

\begin{example}\label{ex:leaf-constraints}
For each leaf node \(i\) we add the constraint:
\begin{gather*}
    n_i = id(\texttt{[0-9]}) \lor n_i = id(\texttt{/}) \lor n_i = id(2) \lor ... \lor n_i = id(10) \lor n_i = id((0,2)) \;\lor \\
    \lor\; n_i = id((1,2)) \lor  n_i = id((0,3)) \lor ... \lor  n_i = id((8,10))\lor  n_i = id((9,10)) 
\end{gather*}
\end{example}


\paragraph{Children constraints.}
If a DSL symbol \(p\) is assigned to a node \(i\), the children of \(i\), \(C(i)\), must have types consistent with the parameters of \(p\).
For each \(p \in \Sigma\) and \(j \in \{1, ..., k\}\), where \(k\) is the largest arity among all DSL constructs, we define \(T(p, j)\).
If \(p\) corresponds to an operator, \(T(p, j)\) denotes the type of parameter \(j\) of \(p\). If \({j > arity(p)}\), then \(T(p,j) = \epsilon\).
If \(p\) represents a literal, then \(T(p,j) = \epsilon\) for every~\(j\).
Finally, let \(\Sigma(T(p,j)) \subset \Sigma\) be the set of terminal symbols in the \ac{DSL} that have type \(T(p,j)\).

\begin{equation}
    \bigwedge_{p \in \Sigma, i \in I}\; \left(n_i = id(p) \Rightarrow \bigwedge_{j \in C(i)} \; \bigvee_{t \in \Sigma(T(p,j))} n_j = id(t) \right)
\end{equation}

\begin{example}\label{ex:children-constraints}
If node 1 is assigned \(\Range\), then its children, nodes 2 and 3, must be assigned symbols of types consistent with its parameters. \({T(\Range, 1) = Re}\), so \(n_2\) must be assigned one of the symbols in
\(\Sigma(Re)=\{\Union, \Concat,\allowbreak \Kleene,\allowbreak \Posit,\allowbreak \Option,\allowbreak \Range, \texttt{[0-9]}, \texttt{/}\}\).
\(T(\Range, 2) = \Rangelit\), so \(n_3\) must be assigned one of the symbols in \(\Sigma(\Rangelit) = \{2,\allowbreak ...,\allowbreak 10,\allowbreak (0,2),\allowbreak (1,2),\allowbreak ... ,\allowbreak (9,10)\}\).
To enforce this, we add the following constraint:
\begin{align*}
    n_1=id(\Range) \Rightarrow (&n_2=id(\Union) \lor n_2=id(\Concat) \lor n_2=id(\Kleene) \,\lor\\
    &\lor n_2=id(\Posit) \lor n_2=id(\Option) \lor n_2=id(\Range) \,\lor\\
    &\lor n_2=id(\texttt{[0-9]}) \lor n_2=id(\texttt{/})\,) \\
    \land \, (&n_3=id(2) \lor ... \lor n_3=id(10) \lor n_3=id((0,2)) \,\lor \\
    &\lor\, n_3=id((1,2)) \lor ... \lor  n_3=id((9,10))\,)
\end{align*}
\end{example}

\paragraph{Output constraints.}  
The root node must be assigned a DSL symbol consistent with the output type. \(Re\) is the desired output type in our DSL. Then \(\Sigma(Re)\) is the set of symbols in the DSL that have type \(Re\).

\begin{equation}
    \bigvee_{p\in \Sigma(Re)} n_1 = id(p)
\end{equation}


\begin{example}
We want or regular expression to have the DSL type \(Re\), so the output constraint for our domain is
\begin{gather*}
    n_1 = id(\Union) \lor n_1 = id(\Concat) \lor n_1 = id(\Kleene) \lor n_1 = id(\Posit) \;\lor \\
    \lor\; n_1 = id(\Option) \lor n_1 = id(\Range) \lor n_1 = id(\texttt{[0-9]}) \lor n_1 = id(\texttt{/})
\end{gather*}
\end{example}

==> tables/double_table.tex <==
\setlength{\dashlinedash}{.5ex}
\setlength{\dashlinegap}{1ex}
\setlength{\tabcolsep}{1ex}


\begin{table}[t]
\caption{Global caption}
\begin{subtable}[t]{.48\linewidth}
\centering
\caption{Comparison of time performance using different synthesis methods.}
\begin{tabular}{@{}lcccc@{}}
    \toprule \small
    \textbf{Timeout (s)}  & \textbf{10} & \textbf{60} & \textbf{3600} \\ \midrule
    \Forest{} (multi-tree)      & 35     & 41     & 48   \\ \hdashline
    Multi-tree w/o pruning      & 27     & 32     & 38   \\
    Dynamic-only multi-tree     & 10     & 15     & 23   \\ \hdashline
    \(k\)-tree                  & 7      & 10     & 17   \\
    Line-based (w/o pruning)    & 4      & 4      & 13   \\ \hdashline
    %10 examples only           & 32     & 42     & 47   \\
    %5 examples only            & 23     & 34     & 44   \\ \midrule
    \Regel{} PBE                & 12     & 16     & 27   \\ \bottomrule
\end{tabular}
\label{table:number-solved}
\end{subtable}%
\begin{subtable}[t]{.48\linewidth}
\centering
\setlength{\tabcolsep}{2ex}
\caption{Comparison of time performance of \Regel{} and \Forest{} on \Regel{}'s Stack Overflow benchmarks.}
\begin{tabular}{@{}lcccc@{}}
    \toprule
    \textbf{Timeout} & \textbf{10} & \textbf{60} & \textbf{3600} \\ \midrule
    \Regel{} PBE               & 63 & 73 & 92 \\
    \Forest{}'s first solution & 34 & 47 & 60 \\
    \Forest{}'s last solution  & 17 & 28 & 50 \\ \bottomrule
\end{tabular}
\label{table:number-solved-resnax}
\end{subtable} 
\end{table}

==> tables/instances_solved_resnax.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{2ex}
\caption{Comparison of time performance of \Regel{} and \Forest{} on \Regel{}'s Stack Overflow benchmarks.}
\begin{tabular}{@{}lcccc@{}}
\toprule
\textbf{Timeout (s)} & \textbf{10} & \textbf{60} & \textbf{3600} \\ \midrule
\Regel{}                   & 63 & 73 & 92 \\
\Forest{}'s first solution & 34 & 47 & 60 \\
\Forest{}'s last solution  & 17 & 28 & 50 \\ \bottomrule
\end{tabular}
\label{table:number-solved-resnax}
\vspace*{-2mm}
\end{table}

